Uncommonly accurate energies for the general quartic oscillator

Recent advances in the asymptotic analysis of energy levels of potentials produce relative errors in eigenvalue sums of order $10^{-34}$, but few non-trivial potentials have been solved numerically to such accuracy. We solve the general quartic potential (arbitrary linear combination of $x^2$ and $x^4$ ) beyond this level of accuracy using a basis of several hundred oscillator states. We list the lowest 20 eigenvalues for 9 such potentials. We confirm the known asymptotic expansion for the levels of the pure quartic oscillator, and extract the next 2 terms in the asymptotic expansion. We give analytic formulas for expansion in up to 3 even basis states. We confirm the virial theorem for the various energy components to similar accuracy. The sextic oscillator levels are also given. These benchmark results should be useful for extreme tests of approximations in several areas of chemical physics and beyond.

==> arXiv/AAWKB.tex <==
\appendix
\sec{Derivation of asymptotic splitting formula}
We now explain how to derive Eq. \ref{AWKB}, the asymptotic approximation to $\D\eps = \eps_1 - \eps_0$ in the limit $\lam \rightarrow \infty$.  

We introduce the shorthand $\eta = (2/\lam)^{3/4}$ so $\lam \rightarrow \infty \implies \eta \rightarrow 0_+$.  In terms of $\eta$ Eq. \ref{CFI} of the main text becomes
\begin{equation}
\label{PhiEta}
\phi(\eta) = \frac{4}{\eta^2} \int_{0}^{\sqrt{1 - \eta}} dx \sqrt{(1 - x^2)^2 - \eta^2}.
\end{equation}
In the limit $\eta \rightarrow 0_+$,
\begin{equation}
\label{ZO}
\phi^{(0)}(\eta) = \frac{4}{\eta^2} \int_{0}^{1} dx (1 - x^2) = \frac{(2 \lam)^{3/2}}{3}.
\end{equation}
We evaluate Eq. \ref{PhiEta}:
\begin{equation}
\label{PhiAnal}
\phi(\eta) = \frac{8}{3 \eta^2} \sqrt{1 + \eta} F(\eta),
\end{equation}
where $F(\eta) = \mathcal{E}(y) - \eta \mathcal{K}(y)$, $y =  (1 - \eta)/(1 + \eta)$ and
\begin{equation}
\mathcal{K}(x) = \int_{0}^{\pi/2} \frac{d\t}{f(x,\theta)}, \hspace{1mm} \mathcal{E}(x) = \int_{0}^{\pi/2} d\t f(x,\theta),
\end{equation}
with $f(x,\theta) = \sqrt{1-x \sin ^2 \t}$ \cite{NIST2}.  The following expansion will prove useful shortly:
\begin{equation}
\label{AsymExpan}
F(\eta) = 1 - \frac{\eta}{2} + \frac{3}{16} \eta^2 (1- 6 \ln 2 + 2 \ln \eta) + \mathcal{O}(\eta^3),
\end{equation}
as $\eta \rightarrow 0_+$ \cite{NIST1}.  Inserting Eq. \ref{AsymExpan} into Eq. \ref{PhiAnal} and expanding around $\eta = 0$, yields
\begin{equation}
\phi^{(2)}(\lam) = \frac{(2 \lam)^{3/2}}{3} - \frac{3}{4} \ln \lam - \frac{1}{4} (2 + 9 \ln2).
\end{equation} 
The above equation combined with Eq. \ref{13} leads to the final result, Eq. \ref{AWKB} of the main text.











